Semantics-based Privacy by Design for Internet of Things Applications

As Internet of Things (IoT) technologies become more widespread in everyday life, privacy issues are becoming more prominent. The aim of this research is to develop a personal assistant that can answer software engineers' questions about Privacy by Design (PbD) practices during the design phase of IoT system development. Semantic web technologies are used to model the knowledge underlying PbD measurements, their intersections with privacy patterns, IoT system requirements and the privacy patterns that should be applied across IoT systems. This is achieved through the development of the PARROT ontology, developed through a set of representative IoT use cases relevant for software developers. This was supported by gathering Competency Questions (CQs) through a series of workshops, resulting in 81 curated CQs. These CQs were then recorded as SPARQL queries, and the developed ontology was evaluated using the Common Pitfalls model with the help of the Prot\'eg\'e HermiT Reasoner and the Ontology Pitfall Scanner (OOPS!), as well as evaluation by external experts. The ontology was assessed within a user study that identified that the PARROT ontology can answer up to 58\% of privacy-related questions from software engineers.

==> CQs_Full_Table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
  \tiny{
\begin{longtable}{p{.001em} p{10em} p{3em} p{3em} p{3em} p{3em} p{14.585em} p{.001em} p{.001em}p{.001em} p{.001em} p{.001em} p{.001em} p{.001em} p{.001em} p{15em} }
  \centering

   {} & {\textbf{CQ}} & {\textbf{Type}} &{\textbf{Sub-type}} & {\textbf{Use case}} & {\textbf{Rank}} & {\textbf{Answer}} & {\begin{sideways}\textbf{Minimize}\end{sideways}} & {\begin{sideways}\textbf{Hide}\end{sideways}} & {\begin{sideways}\textbf{Separate}\end{sideways}} & {\begin{sideways}\textbf{Aggregate}\end{sideways}} & \begin{sideways}\textbf{Inform}\end{sideways} & \begin{sideways}\textbf{Control}\end{sideways} &  {\begin{sideways}\textbf{Enforce}\end{sideways}} & \begin{sideways}\textbf{Demonstrate}\end{sideways} & {\textbf{SPARQL}} \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 1     & What are PbD patterns I should apply if I do not need the identity of the user? (anonymously) & Data Collection & Personal Information & Fitness Watch & Modified & 26.  Pseudonymous Identity &   {X} &       &       &   {X} & {} & {} &       & {} & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:Anonymously ) } \\
    \midrule
    2     & will my clients' data be stored in a secure manner? & Regulations & Agreement & Smart Home & Modified & 4.      Informed Secure Passwords\newline{}32.   Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context &       &       &       &       & X     & X     &       & {} & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:Data\_stored\_securely ) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 3     & What are PbD patterns I should apply  to prevent attackers from identify the identity of the user? & Regulations & Agreement & Fitness Watch & Valid & 2.     Location Granularity\newline{}8.     Use of dummies\newline{}26.  Pseudonymous Identity\newline{}29.  Aggregation Gateway\newline{}44.  Decoupling [content] and Location Information Visibility\newline{}51.  Informed Credential Selection\newline{}55.  Masquerade\newline{}63.  Added-noise measurement obfuscation\newline{}64.  Increasing Awareness of Information Aggregation\newline{}65.  Attribute Based Credentials\newline{}67.  [Support] Selective Disclosure\newline{}73.  Identity Federation Do Not Track Pattern &    {X} &    {X} &    {X} &    {X} & X     & X     &       & X     & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:Hide\_data\_subjects\_identity\_from\_attackers ) } \\
    \midrule
    4     & What are PbD patterns I should apply if my system requires the data subject information e.g., by phone, email, car etc.? & Data Collection & Personal Information & RTLS  & Modified & 3.     Minimal Information Asymmetry\newline{}32.  Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context\newline{}40.  Obtaining Explicit Consent\newline{}41.  Privacy Mirrors\newline{}48.  Privacy Dashboard\newline{}51.  Informed Credential Selection\newline{}54.  Reasonable Level of Control\newline{}58.  Lawful Consent\newline{}61.  Personal Data Table &       &       &       &       & X     & X     &       & X     & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:PersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Email    ?Activity = parrot:Phone) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 5     & What are PbD patterns I should apply if my system shares user's accident information to emergency services & Proccess & Third Party  & Fitness Watch & Valid & 18.  Outsourcing [with consent]\newline{}50.  Obligation Management\newline{}60.  Sticky Policies &       &       &       &       &  {} & X     &  {X} &  {} & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:to\_emergency\_services ) } \\
    \midrule
    6     & What are PbD patterns I should apply to give user privacy notification in case he/she wants to share personal data e.g exact location ? & Proccess & Share & Fitness Watch & Valid & 12.  Discouraging Blanket Strategies\newline{}46.  Selective Access control\newline{}55.  Masquerade\newline{}56.  Buddy List\newline{}67.  [Support] Selective Disclosure\newline{}68.  Private Link &       &       &       &    {X} &  {} & X     &       &  {} & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:user\_to\_user ) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 7     & What are PbD patterns I should apply if my system stores user's daily routine? & Data Collection & Routine & Fitness Watch & Valid & 5.     Awareness Feed.\newline{}8.     Use of dummies\newline{}26.  Pseudonymous Identity\newline{}27.  Personal Data Store\newline{}35.  Enable/Disable Function\newline{}38.  User Data Confinement Pattern \newline{}43.  Impactful Information and Feedback\newline{}48.  Privacy Dashboard\newline{}51.  Informed Credential Selection\newline{}54.  Reasonable Level of Control\newline{}57.  Privacy Awareness Panel\newline{}61.  Personal Data Table\newline{}63.  Added-noise measurement obfuscation\newline{}64.  Increasing Awareness of Information Aggregation\newline{}65.  Attribute Based Credentials &    {X} &    {X} &    {X} &    {X} & X     & X     &       & X     & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Daily\_Routine ) } \\
    \midrule
    8     & What are PbD patterns I should apply if my system requires user's device's properties & Data Collection & Personal Information & Fitness Watch & Valid & 12.  Discouraging Blanket Strategies\newline{}46.  Selective Access control\newline{}55.  Masquerade &       &       &       &    {X} & X     & X     &       &  {} & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Data\_subjects\_device\_properties ) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 9     & What are PbD patterns I should apply if my system stores user's food intake information? & Data Collection & Routine & Fitness Watch & Valid & 5.     Awareness Feed.\newline{}8.     Use of dummies\newline{}26.  Pseudonymous Identity\newline{}27.  Personal Data Store\newline{}35.  Enable/Disable Function\newline{}38.  User Data Confinement Pattern \newline{}43.  Impactful Information and Feedback\newline{}48.  Privacy Dashboard\newline{}51.  Informed Credential Selection\newline{}54.  Reasonable Level of Control\newline{}57.  Privacy Awareness Panel\newline{}61.  Personal Data Table\newline{}63.  Added-noise measurement obfuscation\newline{}64.  Increasing Awareness of Information Aggregation\newline{}65.  Attribute Based Credentials &    {X} &    {X} &    {X} &    {X} & X     & X     &       & X     & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Food\_Data ) } \\
    \midrule
    10    & What are PbD patterns I should apply if my system stores user's gym information? & Data Collection & Personal Information & Fitness Watch & Valid & 26.  Pseudonymous Identity\newline{}27.  Personal Data Store\newline{}35.  Enable/Disable Function\newline{}38.  User Data Confinement Pattern \newline{}43.  Impactful Information and Feedback\newline{}48.  Privacy Dashboard\newline{}51.  Informed Credential Selection\newline{}54.  Reasonable Level of Control\newline{}57.  Privacy Awareness Panel\newline{}61.  Personal Data Table\newline{}64.  Increasing Awareness of Information Aggregation\newline{}65.  Attribute Based Credentials &    {X} &       &    {X} &    {X} & X     & X     &       & X     & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Gym\_Data ) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 11    & What are PbD patterns I should apply if my system scans wireless access points for indoor positioning & Data Collection & Location & Fitness Watch & Valid & 14.  Asynchronous notice\newline{}19.  Ambient Notice\newline{}35.  Enable/Disable Function\newline{}42.  Appropriate Privacy Feedback &       &       &       &       & X     & X     &       & X     & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Indoor\_positioning ) } \\
    \midrule
    12    & recorded sensitive information about customers? & Data Collection & Personal Information & Drone Delivery & Valid & 8.     Use of dummies\newline{}32.  Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context\newline{}63.  Added-noise measurement obfuscation &    {X} &    {X} &       &       & X     & X     &       &  {} & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Sensitive\_personal\_information ) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 13    & has cameras? & Device & Camera & Smart Home & Valid & 14.   Asynchronous notice\newline{}19.   Ambient Notice\newline{}35.   Enable/Disable Function &       &       &       &       & X     & X     &       &  {} & SELECT  ?Device  ?PrivacyPattern\newline{}WHERE { ?Device a parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Device = parrot:Camera ) } \\
    \midrule
    14    & stores address data that belong to previous customers? & Regulations & Agreement & Drone Delivery & Duplicated & 50.  Obligation Management &       &       &       &       & X     &  {} &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ArchiveData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Historical\_Data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 15    & save historical data for how long? & Regulations & Agreement & Drone Delivery & Modified\newline{}Duplicated & 5.     Awareness Feed.\newline{}42.  Appropriate Privacy Feedback\newline{}50.  Obligation Management\newline{}57.  Privacy Awareness Panel &       &       &       &       & X     &  {} &  {X} & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ArchiveData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Historical\_Data) } \\
    \midrule
    16    & requires 24 hour monitoring? & Device & Camera & Drone Delivery & Duplicated & 5.     Awareness Feed.\newline{}9.     Who’s Listening\newline{}14.  Asynchronous notice\newline{}19.  Ambient Notice\newline{}35.  Enable/Disable Function &       &       &       &       & X     & X     &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:24\_Hour\_Monitoring) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 17    & What are the PbD patterns I should apply if the system capabilities such as microphone is always on? & Device & Microphone & Fitness Watch & Valid & 14. Asynchronous notice\newline{}19. Ambient Notice &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Device\_Always\_On) } \\
    \midrule
    18    & What are PbD patterns I should apply if my system allows real-time monitoring of the images locally & Device & Camera & Park Monitoring & Duplicated & 3.     Minimal Information Asymmetry\newline{}14.  Asynchronous notice\newline{}19.  Ambient Notice\newline{}40.  Obtaining Explicit Consent &       &       &       &       & X     & X     &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Live\_Video\_Monitoring) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 19    & provides tracking service? & Data Collection & Location & Drone Delivery & Modified\newline{}Duplicated & 9.     Who’s Listening\newline{}14.  Asynchronous notice\newline{}19.  Ambient Notice\newline{}35.  Enable/Disable Function &       &       &       &       & X     & X     &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Tracking) } \\
    \midrule
    20    & What are PbD patterns I should apply if GPS tracking the car? & Data Collection & Location & RTLS  & Duplicated & 14.  Asynchronous notice\newline{}19.  Ambient Notice\newline{}35.  Enable/Disable Function &       &       &       &       & X     & X     &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Tracking) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 21    & Allows customers to delete their data at any time? & Regulations & Control & Drone Delivery & Modified\newline{}Duplicated & 48.  Privacy Dashboard\newline{}61.  Personal Data Table &       &       &       &       & X     & X     &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Delete\_Data) } \\
    \midrule
    22    & What are PbD patterns I should apply  to allow the user to delete his data if he/she wants to do? & Regulations & Control & Fitness Watch & Duplicated & 48.  Privacy Dashboard\newline{}61.  Personal Data Table &       &       &       &       & X     & X     &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Delete\_Data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 23    & What are PbD patterns I should apply if my system keeps the data for a period of time & Regulations  & Agreement & Fitness Watch & Modified\newline{}Duplicated & 32.  Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context\newline{}40.  Obtaining Explicit Consent\newline{}58.  Lawful Consent\newline{}59.  Privacy Aware Wording &       &       &       &       & X     & X     &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:for\_a\_period\_of\_time) } \\
    \midrule
    24    & What are PbD patterns I should apply  if my system save the videos for long time? & Regulations & Agreement & Park Monitoring & Duplicated & 3.     Minimal Information Asymmetry\newline{}59.  Privacy Aware Wording &       &       &       &       & X     &  {} &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:for\_a\_period\_of\_time) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 25    & What are PbD patterns I should apply if my system stores data in the cloud & Storage & Cloud & Fitness Watch & Duplicated & 8.     Use of dummies\newline{}26.  Pseudonymous Identity\newline{}27.  Personal Data Store\newline{}40.  Obtaining Explicit Consent\newline{}58.  Lawful Consent\newline{}63.  Added-noise measurement obfuscation\newline{}65.  Attribute Based Credentials &    {X} &    {X} &       &    {X} & X     & X     &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:in\_cloud) } \\
    \midrule
    26    & What are PbD patterns I should apply if my system is storing the data in the cloud? & Storage & Cloud & RTLS  & Duplicated & 8.     Use of dummies\newline{}22.  Data Breach Notification Pattern\newline{}27.  Personal Data Store\newline{}41.  Privacy Mirrors\newline{}50.  Obligation Management\newline{}63.  Added-noise measurement obfuscation &    {X} &    {X} &       &       & X     &  {} &  {X} & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:in\_cloud) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 27    & What are PbD patterns I should apply if my system store data in the smart watch? & Storage & Local & Fitness Watch & Modified\newline{}Duplicated & 27.  Personal Data Store\newline{}38.  User Data Confinement Pattern &       &       &    {X} &       & X     &  {} &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Locally) } \\
    \midrule
    28    & What are PbD patterns I should apply if my system can store the data in the mobile? & Storage & Local & Fitness Watch & Modified\newline{}Duplicated & 27.  Personal Data Store\newline{}38.  User Data Confinement Pattern &       &       &    {X} &       & X     &  {} &       & X     & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Locally) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 29    & provides drone access to more than one users (pilots) to provide required services? & Proccess & Access & Drone Delivery & Valid & 5.     Awareness Feed.\newline{}9.     Who’s Listening &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Access\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_service\_provider) } \\
    \midrule
    30    & has the possibility of being infiltrated? & Regulations & Notify & Drone Delivery & Duplicated & 71.  Unusual Activities &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Data\_Infiltration) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 31    & has the possibility of being infiltrated? & Regulations & Notify & Smart Home & Duplicated & 71.  Unusual Activities &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Data\_Infiltration) } \\
    \midrule
    32    & suspects intruder or privacy invasion? & Regulations & Notify & Smart Home & Modified & 22.   Data Breach Notification Pattern\newline{}71.   Unusual Activities &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Intruder) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 33    & was attacked? & Regulations & Notify & Drone Delivery & Modified\newline{}Duplicated & 22.  Data Breach Notification Pattern\newline{}71.  Unusual Activities &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_System\_Attack) } \\
    \midrule
    34    & What are PbD patterns I should apply if my system detects a criminal behaviour? & Regulations  & Notify & Fitness Watch & Duplicated & 22.  Data Breach Notification Pattern\newline{}71.  Unusual Activities &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_System\_Attack) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 35    & What are PbD patterns I should apply if my system have attack/threats? & Regulations  & Notify & Fitness Watch & Duplicated & 22.  Data Breach Notification Pattern\newline{}71.  Unusual Activities &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_System\_Attack) } \\
    \midrule
    36    & What are PbD patterns I should apply if my system can be paired with other IoT devices? & Proccess & Route & RTLS  & Duplicated & 24.  Onion Routing &       &    {X} &       &       &  {} &  {} &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Route\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Between\_Devices) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 37    & connects multiple smart devices and synced data across them? & Proccess & Route & Smart Home & Modified\newline{}Duplicated & 24.   Onion Routing\newline{}35.   Enable/Disable Function &       &    {X} &       &       &  {} & X     &       &  {} & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Route\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Between\_Devices) } \\
    \midrule
    38    & What are PbD patterns I should apply if my system reports data subject’s information to an Administrator/ Controller? & Proccess & Share & Health System & Valid & 9. Who is Listening\newline{}12. Discouraging Blanket Strategies\newline{}26. Pseudonymous Identity\newline{}29. Aggregation Gateway\newline{}69. Anonymity Set &    {X} &    {X} &    {X} &    {X} & X     & X     &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}	WHERE { ?Activity a parrot:Share\_Data.\newline{}		 ?Activity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?Activity = parrot:Report\_for\_Adminstration) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 39    & What are PbD patterns I should apply if my system allows administration staff to view the images & Proccess & Access & Park Monitoring & Valid & 40.  Obtaining Explicit Consent &       &       &       &       &  {} & X     &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE {  \newline{}?Activity rdf:type parrot:Access\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern. \newline{}filter ( ?Activity = parrot:to\_administrator ) } \\
    \midrule
    40    & What are the PbD patterns I should apply if my system allow trusted parties to access my data? & Proccess & Access & Fitness Watch & Valid & 18. Outsourcing [with consent]\newline{}50. Obligation Management\newline{}60. Sticky Policies &       &       &       &       &  {} & X     &  {X} &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE {  \newline{}?Activity rdf:type parrot:Access\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern. \newline{}filter ( ?Activity = parrot:to\_trusted\_parties ) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 41    & What are PbD patterns I should apply if my system collects user's age, gender, marital status and other personal information is required? & Data Collection & Personal Information & Fitness Watch & Modified & 3.     Minimal Information Asymmetry\newline{}26.  Pseudonymous Identity\newline{}27.  Personal Data Store\newline{}32.  Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context\newline{}38.  User Data Confinement Pattern \newline{}40.  Obtaining Explicit Consent\newline{}41.  Privacy Mirrors\newline{}48.  Privacy Dashboard\newline{}51.  Informed Credential Selection\newline{}54.  Reasonable Level of Control\newline{}57.  Privacy Awareness Panel\newline{}61.  Personal Data Table\newline{}64.  Increasing Awareness of Information Aggregation\newline{}65.  Attribute Based Credentials &    {X} &       &    {X} &    {X} & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Collecting\_Personal\_Information) } \\
    \midrule
    42    & What are PbD patterns I should apply if my system is collecting the data continuously? & Data Collection & Routine & RTLS  & Valid & 14.  Asynchronous notice\newline{}19.  Ambient Notice\newline{}42.  Appropriate Privacy Feedback\newline{}70.  Active Broadcast of Presence &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Continuous\_Data\_Collection) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 43    & What are PbD patterns I should apply to make sure non authorised people (staff) accessing the images ? & Regulations & Agreement & Park Monitoring & Modified & 28.  Trust Evaluation of Services Slides\newline{}32.  Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:Compliance.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Non-authorized\_people\_access) } \\
    \midrule
    44    & What are PbD patterns I should apply if my system is being used in different countries applying different privacy policies? & Regulations & Privacy Policy & RTLS  & Valid & 16.  Policy Matching Display\newline{}18.  Outsourcing [with consent]\newline{}21.  Privacy Labels\newline{}30.  Privacy icons\newline{}36.  Privacy Color Coding\newline{}59.  Privacy Aware Wording\newline{}60.  Sticky Policies &       &       &       &       & X     & X     &  {X} & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CrossBorderTransfer.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Used\_in\_Different\_Countries) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 45    & Do I get to choose which data and how much data to be shared across connected devices? & Regulations  & Control & Smart Home & Valid & 35.   Enable/Disable Function\newline{}53.   Negotiation of Privacy Policy\newline{}54.   Reasonable Level of Control &       &       &       &       & X     & X     &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Choose\_Data) } \\
    \midrule
    46    & What are PbD patterns I should apply if my system is processing subject's data? & Proccess & Route & RTLS  & Valid & 24.  Onion Routing\newline{}28.  Trust Evaluation of Services Sides\newline{}38.  User Data Confinement Pattern &       &    {X} &    {X} &       & X     &  {} &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Processing\_Data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 47    & What are the PbD privacy patterns I should apply to allow data subject to choose his collected data? & Regulations  & Control & Health System & Valid & 35. Enable/Disable Function\newline{}45. Platform for Privacy Preferences\newline{}54. Reasonable Level of Control &       &       &       &       & X     & X     &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_chooses\_collected\_data) } \\
    \midrule
    48    & What are PbD patterns I should apply to allow data subject to control his data? & Regulations  & Control & Fitness Watch & Duplicated & 27. Personal Data Store \newline{}35. Enable/Disable Function\newline{}45. Platform for Privacy Preferences\newline{}48. Privacy Dashboard\newline{}54. Reasonable Level of Control &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_controls\_his\_data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 49    & What are the PbD privacy patterns I should apply to allow data subject to have control on his stored data? & Regulations  & Control & Health System & Duplicated & 27. Personal Data Store\newline{}48. Privacy Dashboard &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_controls\_his\_data) } \\
    \midrule
    
    50    & What are PbD patterns I should apply to make sure the data subject has the right to delete his data? & Regulations & Agreement & Park Monitoring & Duplicated & 28.  Trust Evaluation of Services Slides\newline{}32.  Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_deletes\_his\_data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 51    & What are PbD patterns I should apply to ensure data subject’s advantage? & Regulations & advantage & Fitness Watch & Valid & 13. Reciprocity\newline{}17. Incentivized Participation &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Ensure\_data\_subjects\_advantage) } \\
    \midrule
    52    & What are the PbD privacy patterns I should apply if my system requires user login? & Proccess & Profile & Health System & Valid & 4. Informed Secure Passwords\newline{}71. Unusual Activities &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:IdentificationOfDataSubject.\newline{}?Activity parrot:entails ?PrivacyPattern. \newline{}FILTER (?Activity = parrot:Login) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 53    & What are PbD patterns I should apply to ensure my system does not collect data more than what is stated in the privacy policy? & Regulations & Agreement & Fitness Watch & Modified & 28.  Trust Evaluation of Services Slides\newline{}32.  Sign an Agreement to Solve Lack of Trust on the Use of Private Data Context &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ObligationForCollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Specified\_in\_the\_privacy\_policy) } \\
    \midrule
    54    & Requests a consent from data subject to store his data? & Regulations & Agreement & Smart Home & Modified & 15.   Abridged Terms and Condition\newline{}34.   Informed Implicit Consent\newline{}40.   Obtaining Explicit Consent\newline{}58.   Lawful Consent\newline{}59.   Privacy Aware Wording\newline{}62.   Informed Consent for Web-based Transactions &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ObtainingConsent.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Request\_consent\_from\_data\_subject) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 55    & What are the PbD privacy patterns I should apply if my system collects data subject's location? & Data Collection & Location & Health System & Valid & 2. Location Granularity &  {X} &       &       &       &  {} & X     &       &  {} & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern\newline{}FILTER (?Data = parrot:Location) } \\
    \midrule
    56    & What are PbD patterns I should apply if my system store the location in the cloud? & Storage & Cloud & Fitness Watch & Valid & 2.     Location Granularity\newline{}8.     Use of dummies\newline{}44.  Decoupling [content] and Location Information Visibility\newline{}63.  Added-noise measurement obfuscation\newline{}64.  Increasing Awareness of Information Aggregation\newline{}74.  Dynamic Location Granularity &  {X} &  {X} &       &  {X} & X     & X     &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Store\_Location) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 57    & What are PbD patterns I should apply to notify the data subject about his data collection? & Regulations & Notify & Fitness Watch & Valid & 5.     Awareness Feed.\newline{}14. Asynchronous notice\newline{}19. Ambient Notice &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Data\_Collection) } \\
    \midrule
    58    & What are PbD patterns I should apply if my system is notifying the users? & Regulations  & Notify & RTLS  & Valid & 14.  Asynchronous notice\newline{}19.  Ambient Notice &       &       &       &       & X     &  {} &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Users) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 59    & What are PbD patterns I should apply if my system analyse the data in the cloud? (aggregation) & Proccess & Route & Park Monitoring & Modified & 65.  Attribute Based Credentials\newline{}69.  Anonymity Set &  {X} &  {X} &       &  {X} &  {} &  {} &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Route\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_cloud) } \\
    \midrule
    60    & What are PbD patterns I should apply if my system is sending subject's data to the server? & Proccess & Route & RTLS  & Valid & 24.  Onion Routing\newline{}43.  Impactful Information and Feedback &       &  {X} &       &       & X     &  {} &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Route\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_server) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 61    & What are PbD patterns I should apply if my system sell the users info with third parties? & Proccess & Third Party  & Fitness Watch & Valid & 18.  Outsourcing [with consent]\newline{}26.  Pseudonymous Identity\newline{}40.  Obtaining Explicit Consent\newline{}50.  Obligation Management\newline{}54.  Reasonable Level of Control\newline{}58.  Lawful Consent\newline{}60.  Sticky Policies &  {X} &       &       &  {X} &  {} & X     &  {X} & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:sell\_data) } \\
    \midrule
    62    & What are PbD patterns I should apply if my system shares the the collected data between Data subjects? & Proccess & Share & Fitness Watch & Valid & 12. Discouraging Blanket Strategies\newline{}46. Selective Access control\newline{}55. Masquerade\newline{}56. Buddy List\newline{}68. Private Link\newline{}70. Active Broadcast of Presence &       &       &       &  {X} &  {} & X     &       &  {} & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_another\_user) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 63    & What are PbD patterns I should apply if my system store people faces/ photos ( identifiable info) & Storage & Photos & Park Monitoring & Valid & 14.  Asynchronous notice\newline{}19.  Ambient Notice\newline{}40.  Obtaining Explicit Consent &       &       &       &       & X     & X     &       &  {} & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER (?Data = parrot:Face\_photo) } \\
    \midrule
    64    & What are PbD patterns I should apply if my system send raw data ex: people faces? & Data Collection & Personal Information & Park Monitoring & Valid & 38.  User Data Confinement Pattern \newline{}65.  Attribute Based Credentials &  {X} &       &  {X} &  {X} &  {} &  {} &       &  {} & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER (?Data = parrot:Raw\_Data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 65    & What are PbD patterns I should apply if my system keeps user's real-time location in cloud & Data Collection & Location & Fitness Watch & Valid & 5.     Awareness Feed.\newline{}35.  Enable/Disable Function &       &       &       &       & X     & X     &       &  {} & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER (?Data = parrot:Real\_Time\_Location) } \\
    \midrule
    66    & What are the PbD patterns I should apply if the system is collecting/ gathers data subject’s information? & Data Collection & Personal Information & Fitness Watch & Duplicated & 3.     Minimal Information Asymmetry\newline{}5.     Awareness Feed.\newline{}29.  Aggregation Gateway\newline{}38.  User Data Confinement Pattern \newline{}40.  Obtaining Explicit Consent\newline{}42.  Appropriate Privacy Feedback\newline{}43.  Impactful Information and Feedback\newline{}51.  Informed Credential Selection\newline{}57.  Privacy Awareness Panel\newline{}58.  Lawful Consent\newline{}64.  Increasing Awareness of Information Aggregation\newline{}65.  Attribute Based Credentials &  {X} &  {X} &  {X} &  {X} & X     & X     &       & X     & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Collection\_of\_Personal\_Data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 67    & What are PbD patterns I should apply if my system requires collecting Personal Data? & Data Collection & Personal Information & Health System & Duplicated & 1. Protection against Tracking\newline{}2. Location Granularity\newline{}3. Minimal Information Asymmetry\newline{}38. User Data Confinement Pattern\newline{}64. Increasing Aggregation Awareness\newline{}65. Attribute Based Credentials\newline{}66. Trustworthy Privacy Plug-in\newline{}69. Anonymity Set &  {X} &  {X} &  {X} &  {X} & X     & X     &       &  {} & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Collection\_of\_Personal\_Data) } \\
    \midrule
    68    & What are PbD patterns I should apply if my system routes data subject’s information among the system components /nodes? & Proccess & Route & Health System & Valid & 24. Onion Routing\newline{}29. Aggregation Gateway &       &  {X} &  {X} &  {X} &  {} &  {} &       &  {} & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Route\_Data) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 69    & What are PbD patterns I should apply if my system shares data subject’s information with third party. e.g., insurance companies? & Proccess & Third Party  & Fitness Watch & Duplicated & 18. Outsourcing [with consent]\newline{}50. Obligation Management\newline{}60. Sticky Policies &       &       &       &       &  {} & X     &  {X} &  {} & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    70    & What are PbD patterns I should apply if my system shares data subject’s information to a third party/ another organization? & Proccess & Third Party  & Health System & Duplicated & 12. Discouraging Blanket Strategies\newline{}18. Outsourcing [with consent]\newline{}26. Pseudonymous Identity\newline{}29. Aggregation Gateway\newline{}50.   Obligation Management\newline{}58. Lawful Consent\newline{}60. Sticky Policies\newline{}64. Increasing Aggregation Awareness\newline{}69. Anonymity Set &  {X} &  {X} &  {X} &  {X} & X     & X     &  {X} & X     & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 71    & What are PbD patterns I should apply if my system is sharing data subject’s information with third party? & Proccess & Third Party  & RTLS  & Duplicated & 18.  Outsourcing [with consent]\newline{}50.   Obligation Management\newline{}60.  Sticky Policies &       &       &       &       &  {} & X     &  {X} &  {} & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    72    & my TV preferred shows and episodes be shared and accessed by third parties? & Proccess & Third Party  & Smart Home & Modified\newline{}Duplicated & 50.   Obligation Management\newline{}60.   Sticky Policies &       &       &       &       &  {} &  {} &  {X} &  {} & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 73    & What are PbD patterns I should apply if my system \newline{}stores data subject’s information in a cloud-based data base? & Storage & Cloud & Health System & Duplicated & 6. Encryption with User-managed Keys\newline{}8. Use of Dummies\newline{}22. Data Breach Notification Pattern\newline{}27. Personal Data Store\newline{}33. Single Point of Contact\newline{}58. Lawful Consent\newline{}63. Added-noise Obfuscation\newline{}65. Attribute Based Credentials &  {X} &  {X} &       &  {X} & X     & X     &       & X     & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Store\_Data) } \\
    \midrule
    74    & How do you deal with outdoor cameras if they record strangers? & Device & Camera & Smart Home & Valid & 14.   Asynchronous notice\newline{}19.   Ambient Notice &       &       &       &       & X     &  {} &       &  {} & SELECT ?Device  ?PrivacyPattern\newline{}WHERE { ?Device a parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern.\newline{}FILTER (?Device = parrot:Outdoor\_Camera) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 75    & What are PbD patterns I should apply if my system \newline{}includes a user interface/ mobile application/ screen/ mobile phone? & Device & Mobile Phone & Health System & Valid & 10. Privacy Policy Display \newline{}11. Layered Policy Design \newline{}15. Abridged Terms and Conditions\newline{}20. Dynamic Privacy Policy Display\newline{}21. Privacy Labels\newline{}30. Privacy icons\newline{}31. Privacy-Aware Network Client\newline{}36. Privacy Colour Coding\newline{}37. Appropriate Privacy Icons\newline{}39. Icons for Privacy Policies\newline{}59. Privacy Aware Wording &       &       &       &       & X     &  {} &       & X     & SELECT ?Device ?PrivacyPattern\newline{}WHERE {  \newline{}?Device rdf:type parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern. \newline{}filter (?Device = parrot:MobilePhone ) } \\
    \midrule
    76    & records audio when I have a private talk with my home mates? & Device & Microphone & Smart Home & Valid & 5.      Awareness Feed.\newline{}14.   Asynchronous notice\newline{}19.   Ambient Notice\newline{}35.   Enable/Disable Function &       &       &       &       & X     & X     &       &  {} & SELECT ?Device ?PrivacyPattern\newline{}WHERE { ?Device a parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern.\newline{}FILTER (?Device = parrot:Microphone) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 77    & What are PbD patterns I should apply if my system requires user's address & Data Collection & Personal Information & Fitness Watch & Valid & 2.     Location Granularity\newline{}29.  Aggregation Gateway\newline{}38.  User Data Confinement Pattern \newline{}41.  Privacy Mirrors\newline{}48.  Privacy Dashboard\newline{}61.  Personal Data Table\newline{}64.  Increasing Awareness of Information Aggregation\newline{}67.  [Support] Selective Disclosure\newline{}74.  Dynamic Location Granularity &  {X} &  {X} &  {X} &  {X} & X     & X     &       & X     & SELECT ?Personal\_Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Personal\_Data rdf:type gdprtext:PersonalData.\newline{}?Personal\_Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Personal\_Data = parrot:Address ) } \\
    \midrule
    78    & What are PbD patterns I should apply if my system detect age, gender or other properties of customers & Data Collection & Personal Information & Park Monitoring & Valid & 3.     Minimal Information Asymmetry\newline{}40.  Obtaining Explicit Consent\newline{}59.  Privacy Aware Wording\newline{}65.  Attribute Based Credentials\newline{}69.  Anonymity Set &  {X} &  {X} &       &  {X} & X     & X     &       & X     & SELECT ?Personal\_Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Personal\_Data rdf:type gdprtext:PersonalData.\newline{}?Personal\_Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Personal\_Data = parrot:Age ) }\newline{}--\newline{}SELECT ?Personal\_Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Personal\_Data rdf:type gdprtext:PersonalData.\newline{}?Personal\_Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Personal\_Data = parrot:Gender ) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 79    & What are PbD patterns I should apply if my system requires user's city information & Data Collection & Personal Information & Fitness Watch & Valid & 2.     Location Granularity\newline{}29.  Aggregation Gateway\newline{}38.  User Data Confinement Pattern \newline{}41.  Privacy Mirrors\newline{}48.  Privacy Dashboard\newline{}61.  Personal Data Table\newline{}64.  Increasing Awareness of Information Aggregation\newline{}67.  [Support] Selective Disclosure\newline{}74.  Dynamic Location Granularity &  {X} &  {X} &  {X} &  {X} & X     & X     &       & X     & SELECT ?Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Data rdf:type gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Data = parrot:City ) } \\
    \midrule
    80    & What are PbD patterns I should apply if my system includes a Sensor/ device that collects data? & Device & Reading Sensor & Health System & Valid & 14. Asynchronous Notice\newline{}19. Ambient Notice &       &       &       &       & X     &  {} &       &  {} & SELECT ?Sensor  ?PrivacyPattern\newline{}	WHERE { ?Sensor a parrot:Sensor.\newline{}		 ?Sensor parrot:entails ?PrivacyPattern.\newline{}		FILTER (?Sensor = parrot:Glucose\_Sensor) } \\
    \midrule
    \rowcolor[rgb]{ .929,  .929,  .929} 81    & provides cloud access to customers as well? & Proccess & Access & Drone Delivery & Valid & 27.  Personal Data Store\newline{}48.  Privacy Dashboard\newline{}61.  Personal Data Table &       &       &       &       & X     & X     &       & X     & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Access\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_Data\_Subject) } \\
    \bottomrule
    
    \caption{The table shows all data collected and analysed. It shows the CQ, its type and sub-type, the answers and their tags.}
    \label{tab:Data Set}%

\end{longtable}%
}

==> Evaluation_with_OOPS.tex <==
\subsection{Structural Dimension}



% Table generated by Excel2LaTeX from sheet 'Sheet2' Structural Dimension Table

\begin{table}
\tiny{
  \centering
  
\begin{tabular}{ m{9.5em}  m{.01em}  m{7em}  m{15.5em}}
    Pitfall &  & Element  & Fix \\
    \midrule
     {\multirow{3}{9.5em}{ P07. Merging different concepts in the same class.}} & {\multirow{3}{.01em}{3}} &  :Principles\_of\_ Wright\_and\_Raab & {\multirow{3}{15.5em}{The scanner considers these classes to have more than one concept because of the word “and”, however, these names refer to the same PbD scheme.}} \\
          &       & :Pricniples\_of\_ Cavoukian\_and \_Jonas &  \\
         &       & :Goals\_of\_ Rost\_and\_Bock &  \\
   
    \midrule
    {\multirow{3}{9.5em}{P13. Inverse relationships are not explicitly declared.}} & {\multirow{3}{.01em}{3}} & :partially\_inspired \_by & {\multirow{3}{15.5em}{In the PARROT ontology, we did not create an inverse relationship.}} \\
          &       & :fully\_inspired\_by &  \\
          &       & :entails &  \\
    \midrule
    {\multirow{5}{9.5em}{P19. Defining multiple domains or ranges in properties.}} & {\multirow{5}{.01em}{3}} & :partially\_inspired \_by & {\multirow{5}{15.5em}{We addressed this problem by typing the domains and ranges in the “Class expression editor” as a union of/ an intersection of multiple classes as a single domain/ range. }} \\
          &       & :fully\_inspired\_by &  \\
          &       & :entails &  \\
                    &       &  &  \\
                                        &       &  &  \\
    \bottomrule
    \end{tabular}%
    \caption{Structural Dimension Table. The table shows the pitfalls occurred in the OOPS! scanner and how they were assisted.}
  \label{tab:Structural Dimension Table}%
  }
\end{table}%


\begin{figure}
	\centering
	\includegraphics[scale=1]{./figures/structural dimension.png}
	\caption{Structural dimension evaluation result. The screenshot shows the result of evaluating all the reused ontologies; however, we only consider the “parrot” ontology pitfalls.}
    \label{Figure:structural dimension}
\end{figure}





\subsection{Functional Dimension}
\begin{table}
\tiny{
  \centering
  
\begin{tabular}{ m{7.5em}  m{.01em}  m{7.5em}  m{14em}}
    Pitfall &  & Element  & Fix \\
    \midrule
     { P10. Missing disjointness} & {3} &  This pitfall applies to the ontology in general instead of specific elements. & We declared some subclasses of \textit{GDPRtEXT:Principle} and the subclasses of \textit{parrot:Guidline} as disjoint classes. \\
   
    \bottomrule
    \end{tabular}%
    \caption{Functional Dimension Table. The table shows the pitfalls occurred in the OOPS! scanner and how they were assisted.}
  \label{tab:Functional Dimension Table}%
  }
\end{table}%
\begin{figure}
	\centering
	\includegraphics[scale=0.7]{./figures/functional dimension.png}
	\caption{Functional dimension evaluation result. The screenshot shows the result of evaluating all the reused ontologies; however, we only consider the “parrot” ontology pitfalls.}
    \label{Figure:functional dimension}
\end{figure}



\subsection{Functional Dimension}
\begin{table}
\tiny{
  \centering
  
\begin{tabular}{ m{9.5em}  m{.01em}  m{7em}  m{15.5em}}
    Pitfall &  & Element  & Fix \\
    \midrule
     {\multirow{3}{9.5em}{ P07. Merging different concepts in the same class.}} & {\multirow{3}{.01em}{3}} &  :Principles\_of\_ Wright\_and\_Raab & \multirow{3}{15.5em}{This pitfall was solved in the first dimension \ref{tab:Structural Dimension Table}} \\
          &       & :Pricniples\_of\_ Cavoukian\_and \_Jonas &  \\
         &       & :Goals\_of\_ Rost\_and\_Bock &  \\
   
    \midrule
    {\multirow{6}{9.5em}{P08. Missing annotations.}} & {\multirow{6}{.01em}{6}} & PARROT:Sensor & {\multirow{6}{15.5em}{We added annotations to the ontology elements. \ref{tab:Annotations}}} \\
          &       & PARROT:Goal &  \\
          &       & PARROT:Guideline &  \\
          &       & PARROT:Device &  \\
          &       & PARROT:Strategy &  \\
          &       & PARROT:entails &  \\
    \midrule
    {\multirow{3}{9.5em}{P13. Inverse relationships not explicitly declared.}} & {\multirow{3}{.01em}{3}} & :partially\_inspired \_by & {\multirow{3}{15.5em}{This pitfall was addressed in the first dimension. }} \\
          &       & :fully\_inspired\_by &  \\
          &       & :entails &  \\

    \midrule
    {P22. Using different naming conventions in the ontology.} & {This pitfall applies to 
    the ontology in general instead of specific elements.} & & {Because we reused many ontologies, the naming conventions will vary. In the PARROT ontology we use an underscore between the words and capitalize the main words (for example: “$parrot:Principles\_of\_Cavoukian$”). } \\

    \midrule
    {\multirow{3}{9.5em}{P41. No license declared.}} & {\multirow{3}{.01em}{}} & The ontology metadata omits information about the license that applies to the ontology. & {\multirow{3}{15.5em}{ }} \\
    \bottomrule
    \end{tabular}%
    \caption{Usability-Profiling Dimension Table. The table shows the pitfalls occurred in the OOPS! scanner and how they were assisted.}
  \label{tab:Usability-Profiling Dimension Table}%
  }
\end{table}%




%%%%%

% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
\tiny{
  \centering
    \begin{tabular}{rp{9em}p{18.415em}}
          & Elements in PARROT & Annotation \\
    \midrule
    1     & \textit{PARROT:Sensor} & An equivalent class to sosa:Sensor \\
    2     & \textit{PARROT:Privacy\_by\_ Design\_Schemes} & \multicolumn{1}{r}{} \\
    3     & \textit{PARROT:Goal} & A set of Privacy by Design goals created by different parties.  \\
    4     & \textit{PARROT:Guideline} & A set of Privacy by Design guidelines created by different parties. \\
    5     & \textit{PARROT:Device} & The devices used in the system. \\
    6     & \textit{PARROT:Strategy} & A set of Privacy by Design strategies created by different parties. \\
    7     & \textit{PARROT:entails} & The relationship between system components or activities with the privacy patterns.  \\
    8     & \textit{PARROT:fully\_inspired\_by} & Is the relationship between the PbD schemes that indicates the connection between a privacy pattern and the other schemes (Principle, Guideline, and Strategy). This connection indicates a full inspiration for the privacy pattern from the privacy scheme. \\
    9     & \textit{PARROT:partially\_ inspired\_by} & Is the relationship between the PbD schemes that indicates the connection between a privacy pattern and the other schemes (Principle, Guideline, and Strategy). This connection indicates a partial inspiration for the privacy pattern from the privacy scheme. \\
    10    & \textit{PARROT:Privacy\_Pattern} & A set of Privacy by Design privacy patterns created by different parties. This level of Privacy by Design Schemes is linked to all the elements in other Privacy by Design Schemes. It is also linked to systems’ components and activities.  \\
    11    & \textit{GDPRtEXT:Principle} & A set of Privacy by Design principles created by different parties. \\
    12    & \textit{PARROT:Notification\_ Activity} & The activity of notifying the data subject about any activity. \\
    13    & \textit{PARROT:Access\_Data} & The activity of providing access to the data for an individual or an organization. Ex: administrator. \\
    14    & \textit{PARROT:Share\_Data} & The activity of sharing some data subject's information to an individual, a friend or an organization. \\
    15    & \textit{PARROT:Route\_Data} & The activity of routing data among different nodes of the system. \\
    \bottomrule
    \end{tabular}%
    
    \caption{The table shows PARROT elements and the annotation added to them}
  \label{tab:Annotations}%
  }
\end{table}%



\begin{figure}
	\centering
	\includegraphics[scale=0.7]{./figures/Usability-Profiling Dimension.png}
	\caption{Usability-Profiling dimension evaluation result. The screenshot shows the result of evaluating all the reused ontologies; however, we only consider the “parrot” ontology pitfalls.}
    \label{Figure:Usability-Profiling Dimension}
\end{figure}
\subsection{Lexical Semantics Experts Evaluation}


==> ORSD.tex <==
\begin{enumerate} %document numerate
\item \textbf{Purpose}
The purpose of building the PARROT ontology is to combine the knowledge of privacy-preserving schemes and IoT devices for systematic guidance to software developers when designing IoT systems.

\item \textbf{Scope}
The ontology will include the 10 Privacy by Design (PbD) schemes cited in the technical report, IoT knowledge. In addition, it encapsulates the associations of IoT and PbD schemes to answer the competency questions stated in this document.

\item \textbf{Implementation Language}
The ontology must be implemented in the OWL2 language.
 
\item \textbf{Intended End-Users}
User1. Software developers who are intending to apply privacy-preserving practices in the design phase of their systems.
User2. Researchers who are looking for a modeled knowledge of privacy schemes and IoT sensors for different purposes.
 
\item \textbf{Intended Uses}
Use1. For tools that need a semantic knowledge base to get information about applying privacy-preserving practices.
Use2.  For companies and organizations who intend to apply privacy-preserving practices.
 
\item \textbf{Ontology Requirements}
\begin{enumerate} % non-fun and fun requirements
\item Non-Functional Requirements
\begin{enumerate} %non-functional list
\item[] NFR1. The ontology must include all Privacy by Design (PbD) schemes stated in the technical report.
\item[] NFR2. The ontology must include the relationship between the different PbD schemes as stated in the technical report.
\item[] NFR3. The ontology must identify similar PbD schemes.
\item[] NFR4. The ontology must include the IoT components.
\item[] NFR5. The ontology must include the IoT components and their associated Privacy Patterns.
\end{enumerate} 

\item Functional Requirements: Groups of Competency Questions
\begin{enumerate} %%%% Use cases numerate
\item[] \textbf{CQG1. Health System (11 CQ)}
\begin{enumerate} %% CQs sub-list
\item[] CQ1.	What are PbD patterns I should apply if my system includes a user interface/ mobile application/ screen/ mobile phone?
\item[] CQ2.	What are PbD patterns I should apply if my system stores data subject’s information in a cloud-based data base?
\item[] CQ3.	What are PbD patterns I should apply if my system reports data subject’s information to an Administrator/ Controller?
\item[] CQ4.	What are PbD patterns I should apply if my system shares data subject’s information to a third party/ another organization?
\item[] CQ5.	What are PbD patterns I should apply if my system requires collecting Personal Data?
\item[] CQ6.	What are PbD patterns I should apply if my system includes a Sensor/ device that collects data?
\item[] CQ7.	What are PbD patterns I should apply if my system routes data subject’s information among the system components /nodes?
\item[] CQ8.	What are the PbD privacy patterns I should apply if my system requires user login?
\item[] CQ9.	What are the PbD privacy patterns I should apply to allow data subject to have control on his stored data?
\item[] CQ10.	What are the PbD privacy patterns I should apply to allow data subject to choose his collected data?
\item[] CQ11.	What are the PbD privacy patterns I should apply if my system collects data subject's location?

\end{enumerate} %% CQs sub-list
 
 
\item[] \textbf{CQG2. Drone Delivery (10 CQ)}
\begin{enumerate} %% CQs sub-list
\item[] CQ12.	What are PbD patterns I should apply if my system provides tracking service?
\item[] CQ13.	What are PbD patterns I should apply if my system was attacked?
\item[] CQ14.	What are PbD patterns I should apply if my system stores address data that belong to previous customers?
\item[] CQ15.	What are PbD patterns I should apply if my system has the possibility of being infiltrated?
\item[] CQ16.	What are PbD patterns I should apply if my system allows customers to delete their data at any time?
\item[] CQ17.	What are PbD patterns I should apply if my system provides cloud access to customers as well?
\item[] CQ18.	What are PbD patterns I should apply if my system provides drone access to more than one users (pilots) to provide required services?
\item[] CQ19.	What are PbD patterns I should apply if my system requires 24 hour monitoring?
\item[] CQ20.	What are PbD patterns I should apply if my system save historical data for how long?
\item[] CQ21.	What are PbD patterns I should apply if my system recorded sensitive information about customers?
\end{enumerate} %% CQs sub-list


\item[] \textbf{CQG3. Fitness Watch (32 CQ)}
\begin{enumerate} %% CQs sub-list
\item[] CQ22.	What are PbD patterns I should apply to ensure data subject’s advantage?
\item[] CQ23.	What are PbD patterns I should apply to ensure my system does not collect data more than what is stated in the privacy policy?
\item[] CQ24.	What are the PbD patterns I should apply if the system capabilities such as microphone is always on?
\item[] CQ25.	What are PbD patterns I should apply if my system shares data subject’s information with third party. e.g., insurance companies?
\item[] CQ26.	What are the PbD patterns I should apply if my system allow trusted parties to access my data?
\item[] CQ27.	What are the PbD patterns I should apply if the system is collecting/ gathers data subject’s information?
\item[] CQ28.	What are PbD patterns I should apply to notify the data subject about his data collection?
\item[] CQ29.	What are PbD patterns I should apply to allow data subject to control his data?
\item[] CQ30.	What are PbD patterns I should apply if my system detects a criminal behaviour?
\item[] CQ31.	What are PbD patterns I should apply if my system shares the the collected data between Data subjects?
\item[] CQ32.	What are PbD patterns I should apply if my system stores data in the cloud?
\item[] CQ33.	What are PbD patterns I should apply if my system store data in the smart watch?
\item[] CQ34.	What are PbD patterns I should apply if my system keeps user's real-time location in cloud
\item[] CQ35.	What are PbD patterns I should apply if my system store the location in the cloud?
\item[] CQ36.	What are PbD patterns I should apply if my system can store the data in the mobile?
\item[] CQ37.	What are PbD patterns I should apply if my system keeps the data for a period of time?
\item[] CQ38.	What are PbD patterns I should apply if my system sell the users info with third parties?
\item[] CQ39.	What are PbD patterns I should apply if my system collects user's age, gender, marital status and other personal information is required?
\item[] CQ40.	What are PbD patterns I should apply if my system stores user's food intake information?
\item[] CQ41.	What are PbD patterns I should apply if my system stores user's gym information?
\item[] CQ42.	What are PbD patterns I should apply if I do not need the identity of the user? (anonymise)
\item[] CQ43.	What are PbD patterns I should apply  to prevent attackers from identify the identity of the user?
\item[] CQ44.	What are PbD patterns I should apply if my system requires user's city information?
\item[] CQ45.	What are PbD patterns I should apply  to allow the user to delete his data if he/she wants to do?
\item[] CQ46.	What are PbD patterns I should apply if my system requires user's address?
\item[] CQ47.	What are PbD patterns I should apply to give user privacy notification in case he/she wants to share personal data e.g exact location ?
\item[] CQ48.	What are PbD patterns I should apply if my system scans wireless access points for indoor positioning?
\item[] CQ49.	What are PbD patterns I should apply if my system have attack/threats?
\item[] CQ50.	What are PbD patterns I should apply if my system stores user's daily routine?
\item[] CQ51.	What are PbD patterns I should apply if my system requires user's device's properties?
\item[] CQ52.	What are PbD patterns I should apply if my system shares user's accident information to emergency services?
\end{enumerate} %% CQs sub-list 
 
 
 
\item[] \textbf{CQG4. Park Monitoring (10 CQ)}
\begin{enumerate} %% CQs sub-list
\item[] CQ53.	What are PbD patterns I should apply if my system store people faces/ photos ( identifiable info)?
\item[] CQ54.	What are PbD patterns I should apply if my system allows administration staff to view the images?
\item[] CQ55.	What are PbD patterns I should apply to make sure non authorised people (staff) accessing the images?
\item[] CQ56.	What are PbD patterns I should apply if my system send raw data ex: people faces?
\item[] CQ57.	What are PbD patterns I should apply if my system detect age, gender or other properties of customers?
\item[] CQ58.	What are PbD patterns I should apply to make my system analyse (aggregation) the data in the cloud?
\item[] CQ59.	What are PbD patterns I should apply to make sure the data subject has the right to delete his data?
\item[] CQ60.	What are PbD patterns I should apply  if my system save the videos for long time?
\item[] CQ61.	What are PbD patterns I should apply if my system allows real-time monitoring of the images locally?

\end{enumerate} %% CQs sub-list
 
 
 
\item[] \textbf{CQG5. Real-Time Tracking System RTLS (13 CQ)}
\begin{enumerate} %% CQs sub-list
\item[] CQ62.	What are PbD patterns I should apply if my system is storing the data in the cloud?
\item[] CQ63.	What are PbD patterns I should apply if my system is sharing data subject’s information with third party?
\item[] CQ64.	What are PbD patterns I should apply if my system is being used in different countries applying different privacy policies?
\item[] CQ65.	What are PbD patterns I should apply if my system is notifying the users?
\item[] CQ66.	What are PbD patterns I should apply if my system is collecting the data continuously?
\item[] CQ67.	What are PbD patterns I should apply if my system is sending subject's data to the server?
\item[] CQ68.	What are PbD patterns I should apply if my system is processing subject's data?
\item[] CQ69.	What are PbD patterns I should apply if GPS tracking the car?
\item[] CQ70.	What are PbD patterns I should apply if my system requires contacting the data subject e.g., by phone, email, etc.?
\item[] CQ71.	What are PbD patterns I should apply if my system can be paired with other IoT devices?

\end{enumerate} %% CQs sub-list
 
 
 
\item[] \textbf{CQG6. Smart Home (11 CQ)}
\begin{enumerate} %% CQs sub-list
\item[] CQ72.	What are PbD patterns I should apply if the TV preferred shows and episodes be shared and accessed by third parties?
\item[] CQ73.	What are PbD patterns I should apply if my system allows data subject to choose which data and how much data to be shared across connected devices?
\item[] CQ74.	What are PbD patterns I should apply if my system connects multiple smart devices and synced data across them?
\item[] CQ75.	What are PbD patterns I should apply if my system has the possibility of being infiltrated?
\item[] CQ76.	What are PbD patterns I should apply if my system stores clients' data in a secure manner?
\item[] CQ77.	What are PbD patterns I should apply if my system records audio when I have a private talk with my home mates?
\item[] CQ78.	What are PbD patterns I should apply if my system requests a consent from data subject to store his data?
\item[] CQ79.	How do you deal with outdoor cameras if they record strangers?
\item[] CQ80.	What are PbD patterns I should apply if my system suspects intruder or privacy invasion?
\item[] CQ81.	What are PbD patterns I should apply if my system has cameras?
\end{enumerate} %% CQs sub-list


\end{enumerate} % non-fun and fun requirements
\end{enumerate} %%%% Use cases numerate
 
%7.      ﻿Pre-Glossary of Terms
%a.      ﻿Terms from Competency Questions
%b.      ﻿Terms from Answers
%c.       ﻿Objects

\end{enumerate} %document numerate

==> validation.tex <==
 % Table generated by Excel2LaTeX from sheet 'Validation'
\tiny{
    \begin{longtable}{ l p{55.5em}}
    \toprule
    \multicolumn{2}{c}{\textbf{Health Care System}} \\
    \midrule
    CQ1.  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system includes a user interface/ mobile application/ screen/ mobile phone?} \\
\cmidrule{2-2}          & SELECT ?Device ?PrivacyPattern\newline{}WHERE {  \newline{}?Device rdf:type parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern. \newline{}filter (?Device = parrot:MobilePhone ) } \\
    \midrule
    CQ2.  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system stores data subject’s information in a cloud-based data base?} \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Store\_Data) } \\
    \midrule
    CQ3.  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system reports data subject’s information to an Administrator/ Controller?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}	WHERE { ?Activity a gdprtext:SystematicMonitoring.\newline{}		 ?Activity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?Activity = parrot:Report\_for\_Adminstration) } \\
    \midrule
    CQ4.  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system shares data subject’s information to a third party/ another organization?} \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    CQ5.  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system requires collecting Personal Data?} \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Collection\_of\_Personal\_Data) } \\
    \midrule
    CQ6.  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system includes a Sensor/ device that collects data?} \\
\cmidrule{2-2}          & SELECT ?Sensor  ?PrivacyPattern\newline{}	WHERE { ?Sensor a parrot:Sensor.\newline{}		 ?Sensor parrot:entails ?PrivacyPattern.\newline{}		FILTER (?Sensor = parrot:Glucose\_Sensor) } \\
    \midrule
    CQ7.  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system routes data subject’s information among the system components /nodes?} \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Route\_Data) } \\
    \midrule
    CQ8.  & \multicolumn{1}{l}{What are the PbD privacy patterns I should apply if my system requires user login?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:IdentificationOfDataSubject.\newline{}?Activity parrot:entails ?PrivacyPattern. \newline{}FILTER (?Activity = parrot:Login) } \\
    \midrule
    CQ9.  & \multicolumn{1}{l}{What are the PbD privacy patterns I should apply to allow data subject to have control on his stored data?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_controls\_his\_data) } \\
    \midrule
    CQ10. & \multicolumn{1}{l}{What are the PbD privacy patterns I should apply to allow data subject to choose his collected data?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_chooses\_collected\_data) } \\
    \midrule
    CQ11. & \multicolumn{1}{l}{What are the PbD privacy patterns I should apply if my system collects data subject's location?} \\
\cmidrule{2-2}          & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern\newline{}FILTER (?Data = parrot:Location) } \\
    \midrule
    \multicolumn{2}{c}{\textbf{Drone Delivery System}} \\
    \midrule
    CQ12. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system provides tracking service?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Tracking) } \\
    \midrule
    CQ13. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system was attacked?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_System\_Attack) } \\
    \midrule
    CQ14. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system stores address data that belong to previous customers?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ArchiveData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Historical\_Data) } \\
    \midrule
    CQ15. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system has the possibility of being infiltrated?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Data\_Infiltration) } \\
    \midrule
    CQ16. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system has a middle device that provides automated control?} \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    CQ17. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system allows customers to delete their data at any time?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Delete\_Data) } \\
    \midrule
    CQ18. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system provides cloud access to customers as well?} \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    CQ19. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system provides drone access to more than one users (pilots) to provide required services? } \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Access\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_service\_provider) } \\
    \midrule
    CQ20. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system requires 24 hour monitoring?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:24\_Hour\_Monitoring) } \\
    \midrule
    CQ21. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system save historical data for how long?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ArchiveData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Historical\_Data) } \\
    \midrule
    CQ22. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system recorded sensitive information about customers?} \\
\cmidrule{2-2}          & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Sensitive\_personal\_information ) } \\
    \midrule
    \multicolumn{2}{c}{\textbf{Fitness Watch}} \\
    \midrule
    CQ23. & \multicolumn{1}{l}{What are PbD patterns I should apply to ensure data subject’s advantage?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Ensure\_data\_subjects\_advantage) } \\
    \midrule
    CQ24. & \multicolumn{1}{l}{What are PbD patterns I should apply to ensure my system does not collect data more than what is stated in the privacy policy?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ObligationForCollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Specified\_in\_the\_privacy\_policy) } \\
    \midrule
    CQ25. & \multicolumn{1}{l}{What are the PbD patterns I should apply if the system capabilities such as microphone is always on?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Device\_Always\_On) } \\
    \midrule
    CQ26. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system shares data subject’s information with third party. e.g., insurance companies?} \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    CQ27. & \multicolumn{1}{l}{What are the PbD patterns I should apply if my system allow trusted parties to access my data?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE {  \newline{}?Activity rdf:type parrot:Access\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern. \newline{}filter ( ?Activity = parrot:to\_trusted\_parties ) } \\
    \midrule
    CQ28. & \multicolumn{1}{l}{What are the PbD patterns I should apply if the system is collecting/ gathers data subject’s information?} \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Collection\_of\_Personal\_Data) } \\
    \midrule
    CQ29. & \multicolumn{1}{l}{What are PbD patterns I should apply to notify the data subject about his data collection?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Data\_Collection) } \\
    \midrule
    CQ30  & \multicolumn{1}{l}{What are PbD patterns I should apply to allow data subject to control his data?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_controls\_his\_data) } \\
    \midrule
    CQ31. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system detects a criminal behaviour?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_System\_Attack) } \\
    \midrule
    CQ32. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system shares the the collected data between Data subjects?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_another\_user) } \\
    \midrule
    CQ33. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system stores data in the cloud?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:in\_cloud) } \\
    \midrule
    CQ34. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system store data in the smart watch? } \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Locally) } \\
    \midrule
    CQ35. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system keeps user's real-time location in cloud?} \\
\cmidrule{2-2}          & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER (?Data = parrot:Real\_Time\_Location) } \\
    \midrule
    CQ36. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system store the location in the cloud? } \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Store\_Location) } \\
    \midrule
    CQ37. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system can store the data in the mobile? } \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Locally) } \\
    \midrule
    CQ38. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system keeps the data for a period of time?} \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:for\_a\_period\_of\_time) } \\
    \midrule
    CQ39  & \multicolumn{1}{l}{What are PbD patterns I should apply if my system sell the users info with third parties? } \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:sell\_data) } \\
    \midrule
    CQ40. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system collects user's age, gender, marital status and other personal information is required?} \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Collecting\_Personal\_Information) } \\
    \midrule
    CQ41. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system stores user's food intake information? } \\
\cmidrule{2-2}          & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Food\_Data ) } \\
    \midrule
    CQ42. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system stores user's gym information? } \\
\cmidrule{2-2}          & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Gym\_Data ) } \\
    \midrule
    CQ43. & \multicolumn{1}{l}{What are PbD patterns I should apply if I do not need the identity of the user? (anonymously) } \\
\cmidrule{2-2}          & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:Anonymously ) } \\
    \midrule
    CQ44. & \multicolumn{1}{l}{What are PbD patterns I should apply  to prevent attackers from identify the identity of the user? } \\
\cmidrule{2-2}          & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:Hide\_data\_subjects\_identity\_from\_attackers ) } \\
    \midrule
    CQ45. & \multicolumn{1}{l}{What are PbD patterns I should apply if my system requires user's city information?} \\
\cmidrule{2-2}          & SELECT ?Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Personal\_Data rdf:type gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Data = parrot:City ) } \\
    \midrule
    CQ46. & \multicolumn{1}{l}{What are PbD patterns I should apply  to allow the user to delete his data if he/she wants to do? } \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Delete\_Data) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ47.} & What are PbD patterns I should apply if my system requires user's address? \\
\cmidrule{2-2}          & SELECT ?Personal\_Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Personal\_Data rdf:type gdprtext:PersonalData.\newline{}?Personal\_Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Personal\_Data = parrot:Address ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ48.} & What are PbD patterns I should apply to give user privacy notification in case he/she wants to share personal data egexact location? \\
\cmidrule{2-2}          & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:user\_to\_user ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ49.} & What are PbD patterns I should apply if my system scans wireless access points for indoor positioning? \\
\cmidrule{2-2}          & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Indoor\_positioning ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ50.} & What are PbD patterns I should apply to give the right access to the mobile app/ desktop website?  \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ51.} & What are PbD patterns I should apply if my system have attack/threats?  \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_System\_Attack) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ52.} & What are PbD patterns I should apply if my system stores user's daily routine?  \\
\cmidrule{2-2}          & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Daily\_Routine ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ53.} & What are PbD patterns I should apply if my system requires user's device's properties? \\
\cmidrule{2-2}          & SELECT  ?Data  ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Data = parrot:Data\_subjects\_device\_properties ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ54.} & What are PbD patterns I should apply if my system shares user's accident information to emergency services? \\
\cmidrule{2-2}          & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Share\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:to\_emergency\_services ) } \\
    \midrule
    \multicolumn{2}{c}{\textbf{Park Monitoring System}} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ55.} & What are PbD patterns I should apply if my system store people faces/ photos ( identifiable info)? \\
\cmidrule{2-2}          & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER (?Data = parrot:Face\_photo) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ56.} & What are PbD patterns I should apply if my system allows administration staff to view the images? \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE {  \newline{}?Activity rdf:type parrot:Access\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern. \newline{}filter ( ?Activity = parrot:to\_administrator ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ57.} & What are PbD patterns I should apply to make sure non authorised people (staff) accessing the images?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:Compliance.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Non-authorized\_people\_access) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ58.} & What are PbD patterns I should apply if my system send raw data ex: people faces?  \\
\cmidrule{2-2}          & SELECT ?Data ?PrivacyPattern\newline{}WHERE { ?Data a gdprtext:PersonalData.\newline{}?Data parrot:entails ?PrivacyPattern.\newline{}FILTER (?Data = parrot:Raw\_Data) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ59.} & What are PbD patterns I should apply if my system detect age, gender or other properties of customers  \\
\cmidrule{2-2}          & SELECT ?Personal\_Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Personal\_Data rdf:type gdprtext:PersonalData.\newline{}?Personal\_Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Personal\_Data = parrot:Age ) }\newline{}--\newline{}SELECT ?Personal\_Data ?PrivacyPattern\newline{}WHERE {  \newline{}?Personal\_Data rdf:type gdprtext:PersonalData.\newline{}?Personal\_Data parrot:entails ?PrivacyPattern. \newline{}filter ( ?Personal\_Data = parrot:Gender ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ60.} & What are PbD patterns I should apply to make my system analyse the data in the cloud? (aggregation) \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Route\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:to\_cloud) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ61.} & What are PbD patterns I should apply to make sure the data subject has the right to delete his data?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Data\_subject\_deletes\_his\_data) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ62.} & What are PbD patterns I should apply  if my system save the videos for long time?  \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:for\_a\_period\_of\_time) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ63.} & What are PbD patterns I should apply if my system allows real-time monitoring of the images locally? \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Live\_Video\_Monitoring) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ64.} & What are PbD patterns I should apply if my system stores my provided personal information in relation with images?  \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    \multicolumn{2}{c}{\textbf{Real-Time Tracking System RTLS}} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ65.} & What are PbD patterns I should apply if my system is storing the data in the cloud?  \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:StoreData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:in\_cloud) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ66.} & What are PbD patterns I should apply if my system is sharing data subject’s information with third party?  \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ67.} & What are PbD patterns I should apply if my system is being used in different countries applying different privacy policies?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CrossBorderTransfer.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Used\_in\_Different\_Countries) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ68.} & What are PbD patterns I should apply if my system is notifying the users?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Users) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ69.} & What are PbD patterns I should apply if my system is collecting the data continuously?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Continuous\_Data\_Collection) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ70.} & What are PbD patterns I should apply if my system is sending subject's data to the server?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern
\newline{}
WHERE { ?Activity a parrot:Route\_Data.
\newline{}?Activity parrot:entails ?PrivacyPattern.
\newline{}FILTER (?Activity = parrot:to\_server) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ71.} & What are PbD patterns I should apply if my system is processing data subject’s information on the server?  \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ72.} & What are PbD patterns I should apply if my system is processing subject's data?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Processing\_Data) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ73.} & What are PbD patterns I should apply if GPS tracking the car?  \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:CollectionOfPersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Tracking) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ74.} & What are PbD patterns I should apply if my system is used in a personal location, e.g. home, car, office?  \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ75.} & What are PbD patterns I should apply if my system requires contacting the data subject e.g., by phone, email, etc.?  \\
\cmidrule{2-2}          & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:PersonalData.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Email || ?Activity = parrot:Phone) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ76.} & What are PbD patterns I should apply if my system can be accessed on more than one device?  \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ77.} & What are PbD patterns I should apply if my system can be paired with other IoT devices? \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Route\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Between\_Devices) } \\
    \midrule
    \multicolumn{2}{c}{\textbf{Smart Home System}} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ78.} & What are PbD patterns I should apply if the TV preferred shows and episodes be shared and accessed by third parties?  \\
\cmidrule{2-2}          & SELECT ?DataActivity ?PrivacyPattern\newline{}	WHERE { ?DataActivity a gdprtext:DataActivity.\newline{}		 ?DataActivity parrot:entails ?PrivacyPattern.\newline{}		FILTER (?DataActivity = parrot:Share\_Personal\_Data\_with\_Third\_Party) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ79.} & What are PbD patterns I should apply if my system allows data subject to choose which data and how much data to be shared across connected devices?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:DataActivity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Choose\_Data) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ80.} & What are PbD patterns I should apply if my system connects multiple smart devices and synced data across them?  \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Route\_Data.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Between\_Devices) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ81.} & What are PbD patterns I should apply if my system has the possibility of being infiltrated?  \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Data\_Infiltration) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ82.} & What are PbD patterns I should apply if my system stores clients' data in a secure manner?  \\
\cmidrule{2-2}          & SELECT  ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ExerciseRights.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Activity = parrot:Data\_stored\_securely ) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ83.} & How PbD deal with my image? e.g., where will they be stored and for how long?  \\
\cmidrule{2-2}          & \multicolumn{1}{l}{} \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ84.} & What are PbD patterns I should apply if my system records audio when I have a private talk with my home mates?  \\
\cmidrule{2-2}          & SELECT ?Device ?PrivacyPattern\newline{}WHERE { ?Device a parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern.\newline{}FILTER (?Device = parrot:Microphone) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ85.} & What are PbD patterns I should apply if my system requests a consent from data subject to store his data?  \\
\cmidrule{2-2}          & SELECT ?Activity ?PrivacyPattern\newline{}WHERE { ?Activity a gdprtext:ObtainingConsent.\newline{}?Activity parrot:entails ?PrivacyPattern\newline{}FILTER (?Activity = parrot:Request\_consent\_from\_data\_subject) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ86.} & How do you deal with outdoor cameras if they record strangers?  \\
\cmidrule{2-2}          & SELECT ?Device  ?PrivacyPattern\newline{}WHERE { ?Device a parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern.\newline{}FILTER (?Device = parrot:Outdoor\_Camera) } \\
    \midrule
    \multicolumn{1}{p{4em}}{CQ87.} & What are PbD patterns I should apply if my system suspects intruder or privacy invasion?  \\
\cmidrule{2-2}          & SELECT ?Activity  ?PrivacyPattern\newline{}WHERE { ?Activity a parrot:Notification\_Activity.\newline{}?Activity parrot:entails ?PrivacyPattern.\newline{}FILTER (?Activity = parrot:Notify\_Intruder) } \\

    \midrule
    \multicolumn{1}{p{4em}}{CQ88.} & What are PbD patterns I should apply if my system has cameras?  \\
\cmidrule{2-2}          & SELECT  ?Device  ?PrivacyPattern\newline{}WHERE { ?Device a parrot:Device.\newline{}?Device parrot:entails ?PrivacyPattern.\newline{}FILTER ( ?Device = parrot:Camera ) } \\
    \bottomrule
    
    
    
    \caption{The PARROT ontology validation via SPARQL queries. The table shows the CQs grouped regarding the use cases and thier SPARQL queries.}
\label{tab:Validation}%

\end{longtable}%
}

